Enabling Information Centric Networks through Opportunistic Search, Routing and Caching

Content dissemination networks are pervasive in todays Internet. Examples of content dissemination networks include peer-to-peer networks (P2P), content distribution networks (CDN) and information centric networks (ICN). In this paper, we propose a new system design for information centric networks which leverages opportunistic searching, routing and caching. Our system design is based on an hierarchical tiered structure. Random walks are used to find content inside each tier, and gateways across tiers are used to direct requests towards servers placed in the top tier, which are accessed in case content replicas are not found in lower tiers. Then, we propose a model to analyze the system in consideration. The model yields metrics such as mean time to find a content and the load experienced by custodians as a function of the network topology. Using the model, we identify trade-offs between these two metrics, and numerically show how to find the optimal time to live of the random walks.

==> background.tex <==
\chapter{Information Centric Networks}
\label{chapt:icn}
 
In this chapter, we present several Information Centric Network proposals encountered in the literature.
We first present DONA, an effort to illustrate drawbacks related to name resolution systems.
We classify the remainder proposals into two groups: $(i)$ distributed hash table proposals and $(ii)$
bread crumb proposals. We focus on the drawbacks related to publish/subscribe and content distribution issues
in both groups, and by the end of this chapter, present guidelines towards an effort to enhance the ICN design. 
The terminology used in the rest of this proposal is presented in Table~\ref{terminology}.  
Figure~\ref{tabproposals} summarizes some of the key features of the ICN proposals discussed in this chapter.


\vspace{0.1in}

\begin{table}[h!]
\center
\begin{tabular}{l|l}
\hline
\textbf{term} & \textbf{description} \\
\hline
\hline
content-data & data stored within the network \\
content-name &  unique name identifier for each content-data \\ 
lookup-request & request for content-data issued by a user \\
locator &  pointer towards content-data storage places \\
cache-router & router able to cache content-data \\
\hline
\end{tabular}
\caption{Table of notation}
\label{terminology}
\end{table}

 
\begin{figure}
\center
\includegraphics[scale=0.6]{proposal}
\label{tabproposals}
\caption{ICN proposals}
\end{figure}


\section{DONA}

DONA ~\cite{dona} is a content distribution solution which embraces ideas built on top of the 
TRIAD ~\cite{triad}, HIP ~\cite{hip} and SFS ~\cite{sfs} proposals. 
DONA adopts a route-by-name to the closest copy approach. Content names are flat. A set of 
\emph{resolution handlers} (RH), used to bind names to locations, are disposed in the network according to an hierarchical tree. Each domain 
has one logical RH, but might have  many physical instances. The use of flat names makes content identification by users
harder (e.g. $m$-bit identifier for each name). It is expected that users obtain the flat names for desired content-data 
through an external mechanism, such as a \emph{search engine}. To provide high-availability, the name resolution process should: 
$(i)$ forward lookup-requests to nearby copies of content-data, and $(ii)$ avoid failed or overloaded servers. 

\begin{figure}[h!]
\center
\includegraphics[scale=0.35]{fig2_1}
\caption{DONA Proposal}
\label{donasystem}
\end{figure}


Each RH stores information for all the contents published in its descendant RHs. 
Since DONA employs flat content-names, not considering name aggregation, a 
single \emph{logical RH} at the top level domain of the hierarchy imposes severe scalability problems. How
the different physical instances of RHs are interconnected, within a given hierarchical level, is left as an open issue.
Figure~\ref{donasystem} illustrates a lookup-request flowing through a set of resolution handlers disposed according to a structured
two level tree. A pointer location to the requested content-data is stored at the logical 
resolution handler in the second level. Content-data flows through a TCP/IP connection towards the user who submitted
the lookup-request. 






\section{Distributed Hash Table Systems}


A distributed hash table (DHT) is a hash table distributed among a dynamic set of participating
nodes. The hash space is subdivided into subsets partitions, with no intersection among them. 
Each partition is managed by one node.  Nodes are identified by a hash-prefix $id$ in the same range of the hashing key-space. 
DHT might be flat or hierarchical, comprising \emph{tiers}~\cite{canon}.  In DHT systems, both lookup-requests 
and content-data are routed according to a structured geometry topology. 


Hash-keys are obtained by applying a hash function to the content-ids.  In some cases, the hash-keys might be the content-ids themselves.
 Lookup-requests 
and content-data are forwarded by the network based on a key-based routing strategy. Once a message \emph{push($k$, content-data)} 
is sent to any node participating in the DHT, the message is forwarded from node to 
node through the network, until encountering the node in charge for hash key $k$. The content will be stored at this node. Each node has an $id$ is responsible for a a set of 
keys.  If a node with identification $id$ is responsible for key $k$, we also say that such a node has an $id$ that owns key $k$.
 Each node will have either a node $id$ that owns $k$, 
or a link to a node whose node $id$ is closer to $k$. 


To get content-data associated with the hash-key $k$, a message \emph{pop($k$)} 
is sent and routed through the network until reaching a node whose node $id$ owns $k$, which will then reply with the stored content-data. 
Each node maintains a set of links to other nodes, its neighbors. Trees, hypercubes and rings are examples of geometries. 
DHT-based systems can guarantee that any data object is located/delivered using at most $O(\log N)$ hops on average, where $N$ 
is the number of nodes in the system. 


An example of a DHT architecture, based on a ring geometry is presented in Figure~\ref{systemdhticn}. In this example, the hash key  
has 8 bits and the hash partition has 2 bits. A user sends a 
lookup-request for content-id 11011011, through the node of the ring identified by the hash-prefix $id$ 00. The lookup-request is 
then sent to the successor node identified by the hash-prefix $id$ 10, before reaching the node $id$ 11. This node is responsible for managing 
the partition where the corresponding content-data for content-id 11011011 is stored at.


\begin{figure}
\center
\includegraphics[scale=0.35]{fig2_2}
\caption{ICN with DHT, ring geometry, 8-bit hash key, 2-bit partition set}
\label{systemdhticn}
\end{figure}


Although DHT search overhead is small, the maintenance overhead might be large in case of node failures/repairs.  
Whenever a node fails or becomes repaired, requests must be sent along the network to reassure the node location in the network.
Neighborhood adjacencies must be reestablished and also, file-index databases related to a partition management must be resettled 
~\cite{dhtmanagement}. 



DHT structures might suffer from reliability flaws 
caused by malicious nodes participating in the DHT and not behaving according to how the protocols were originally set ~\cite{securitydht}.
In particular, DHTs are prone to Sybil attacks and Eclipse attacks. For instance, if a node responsible for managing
the content-data related to a partition misbehaves, all the information for that partition cannot be safeguarded.



PSIRP ~\cite{psirp}, MDHT/Netinf ~\cite{mdht} and MCACHE  ~\cite{multicache} are examples of ICN proposals relying on DHT. 
In the next subsections, publish/subscribe and content distribution issues are discussed in light of these proposals, . 
In DHT proposals, \emph{names} are non-human readable, but can be aggregated according to hash prefixes.  
Both PSIRP and MDHT/Netinf use name resolution systems, whereas MCACHE does not.


\subsection{Publish/Subscribe Issues in DHTs}

In MDHT/Netinf and PSIRP, publications and subscriptions are forwarded to a name resolution system (NRS),
organized according a multi-level hierarchical DHT structure. In PSIRP, the NRS is called \emph{rendezvous}.  
One big advantage of MDHT/Netinf and PSIRP, to DONA's proposal, is that different name resolution servers at the same hierarchical level 
can support name resolution instead of only one logical resolution server per hierarchical level. Each partition of the hash space in a level 
is assigned to a different node server. 


The highest levels of the hierarchy must be highly scalable due to the large number of globally available data objects. 
Failures or performance issues in the top levels might affect a large number of nodes in the network.  MDHT/Netinf claims also that for security reasons, published information should be managed on systems under the control of 
publisher trusted authorities. Interconnecting all nodes through an structure at top level hierarchies would hamper the deployment
of selected trusted authorities by the publishers. MDHT/Netinf proposes that hierarchical top levels name resolution servers should be
disposed in a Global Name Resolution (REX), managed by third parties. The REX would be connected with lower DHT hierarchical levels,
managed by local trusted authorities. The design of robust and scalable REX systems is an important open problem. 



\subsection{Content Distribution Issues in DHTs}


In MDHT/Netinf and PSIRP, all replicas are registered at the NRS. To reduce the overhead on the NRS, the replication policies should not
change cache content too frequently. Finding the right frequency at which to update cache content is an important open problem. 
Another issue regarding NRS is the delay between object placement and NRS synchronization ~\cite{netinf}.


In MCACHE, a rendezvous point is assigned to each published content-data.  This rendezvous point  becomes the root node of
a multicast tree, established along the routers. The same DHT tree structure for routing lookup-requests routes
content-data. The tree structure allows the building of the multicast trees for content-data delivery. 
A copy of each content-data, sent through a multicast tree, is stored at the closest
cache-router connected to the subscribers. 


Lookup-requests issued by the subscribers may be serviced by cached copies.  
Nonetheless, since 
caching of content is restricted to occur at cache-routers close to requesters,
  the limited storage space on such cache-routers might lead to frequent content replacements.
The maintenance of fresh pointers in the network in light of such frequent updates remains a challenge to be addressed.



\begin{comment}
These frequent replacements, in turn, might cause pointers to such contents, stored in other routers in the network, to rapidly stale. 
so to allow the discovery of such copies can point to copies that have already been replaced at those caches,
by newer copies, because of 
\end{comment}




\section {Bread crumb Systems}

Bread crumb (BC) systems are ICN approaches that performs content-id routing at each router without a fixed geometry topology. 
It is assumed that each router knows how to forward lookup requests, based on named-content tables. BC ~\cite{elisha2}, BC+ ~\cite{bc+}
and CCN ~\cite{ccn1} are examples of bread crumb systems. CCN relies on routing protocols to fill and set up named-content tables, 
whereas BC and BC+ do not specify how to fill those tables. Content-data, when sent to subscribers, may be stored as 
replicas in the cache-routers.  


Figure ~\ref{systemicnbread} shows a lookup-request being routed by its name according to named-content tables in routers. 
The names 
can be either human readable names or non-human readable names. When a user sends a lookup-request, the request carries
a content-id of the desired content. The routers forwards the request until a replica of
the content is reached and stores the request itself as a bread crumb, while the request is forwarded. 
The set of bread crumbs of a given request compose
a trail, represented by the green arrows in the figure. Once found, content-data follows the trail of bread crumbs
in the reverse path, until being delivered to the user that issued the content subscription. The path followed
by content-data is illustrated by the blue arrows.


\begin{figure}
\center
\includegraphics[scale=0.35]{fig2_3}
\caption{ICN with bread crumbs}
\label{systemicnbread}
\end{figure}



\subsection{Publish/Subscribe Issues in Bread crumb Systems}


\begin{comment}
The lookup requests are directed towards the nearest copy stored in the network, according to some metric 
at named-content tables. \eat{Lookup-requests carry content-ids composed of human readable names. Those } Content names are used
by the routers, to forward the requests according to information contained in routing-tables. As lookup-requests are forwarded, they are stored at 
the routers as a bread crumbs, which implies lookup-requests leaving a trail of bread crumbs from the subscriber up to 
the corresponding content-data storage location. Content-data is delivered in the reverse path of bread crumbs.

\end{comment}

Lookup requests are routed towards publicly known sources of  content-data. 
Nevertheless, while being forwarded, it may encounter a router wherein a bread crumb for that content-data
is already stored. In this case, following a previously established trail of bread crumbs for that content-data might be more efficient than 
retrieving data from  the publicly 
known source.  For this reason, the lookup request can then be alternatively routed towards an alternative subscriber,
through the bread crumb trail, in an attempt to find a replica of the file. 



According to BC and BC+, bread crumbs are guidance information for the location of content caches,
being designed with the purpose of reducing the load at storage locations (publishers).
An important issue comprising bread crumbs relies on the possibility that some lookup requests, 
when being forwarded towards cached replicas, cannot reach the intended content-data,
due to content-data not existing in the cache anymore. BC+ uses different techniques from BC, 
in order to enhance the probability of lookup requests finding replicas in caches. BC and BC+ leave a number of open 
issues, such as how the named-routing tables should be filled when content-data is published.

\eat{ (*obs to be shown difference between BC and BC+). }




\subsection{Content Distribution Issues in Bread Crumb Systems}


In Bread Crumb systems, content-data is sent to subscribers in the reverse path of bread crumb trails and  
 can be replicated as it is forwarded to users. Content-named-tables can be updated on the fly as content-data 
is sent to subscribers. In CCN, which adopts human readable names, an extension of IP routing protocols, such as OSPF and IS-IS, are proposed for intra-domain routing.  This extension determines how to populate named-content tables in the routers. For inter-domain routing ($i.e.,$ if a router in parc.com domain would like to obtain content 
with the prefix mit.edu), CCN proposes an extension of BGP, another IP network routing protocol, which can also determine how to populate the
named-content tables. 


In general, content-data replicas will not be stored in the domain they were originally published. 
To be encountered, all replicas should be announced by routing protocols in CCN referenced by their global names.  
Avoiding an  explosion of routing table sizes is an important challenge. Assuming published data-content are announced in routing tables only  through their prefixes, an estimate of the number of name prefixes that need to be supported is given by the number of second-level domains 
in the Domain Name System. This number was around 110 million in 2010 ~\cite{netinf}. 





\section{Summary of Open Problems and System Design Guidelines}

\label{sec:summaryopendesign}


Next, we introduce the main guidelines of our system design in light of the background introduced in this chapter.
  Our guidelines target two aspects of ICNs, namely the name resolution system and load balancing.

\begin{itemize}
\item \textbf{Name resolution system (NRS): }  
based on our discussion so far, it should be clear that the NRS  of an ICN 
should be distributed.  Gathering global knowledge about all content-data replicated in the network is 
very difficult, maybe infeasible (see~\textsection\ref{sec:motivation}).  
Also, trying to maintain distributed knowledge in the network, 
in the absence of a NRS, is difficult due to maintainability overheads  
and attacks that could disrupt pre-defined policies (see~\textsection\ref{envisioned}). Another important consideration concerns their
 published content being managed by trusted parties. \emph{A global single structured NRS fully 
connected would need to count only with trusted parties.  }
\item \textbf{Load balancing: }  
Bread crumbs proposals consider load balance policies for replicas of a given 
content over cache routers. 
Nevertheless, the cached replicas are not advertised to the neighborhood of the cache-router where it is stored.
  The information about the replicas is restricted only to the cache routers that the content-data traversed, when sent to users.
\emph{None of the proposals reviewed presents a deeper analysis on the load supported 
by the servers that store published content without disrupting service capacity for solving names 
in name resolution systems. }
\end{itemize}



In this thesis proposal, we devise a solution based on 1) \emph{a tiered architecture}, whereas
 separate \emph{storage areas} are dedicated to different published content, and 2) 
\emph{randomized algorithms} to search for published content across the tiers. 

\begin{enumerate}
\item \textbf{tiered architecture and storage areas: }  we propose randomized  algorithms to encounter popular 
contents in cache routers, in an effort to reduce the searching load in the storage areas. 
Note that we assume that the nodes in a storage areas are not connected according to any pre-established structure or topology. 
\item \textbf{random walks for search and load balance: } random walks have been proposed as a key algorithm
to  address 
topology search/maintenance in peer-to-peer (P2P) networks~\cite{nearoptimal}.
Nevertheless, to the best of our knowledge, previous work in the realm of Information Centric Networks  
has not considered the adoption of  randomized  algorithms for content discovery and replication. 
\end{enumerate}


Randomization is useful for solving complex problems in various applications ~\cite{mitzenmatcher}.  
Two principles at the heart of random algorithms are strongly linked to our investigation~\cite{motwani} are,
\begin{enumerate}
\item \textbf{foil the adversary:} while an adversary may be able to construct an input that foils a
deterministic algorithm, it is difficult to devise an algorithm that can defeat a
random algorithm. Foil the adversary is a key point to avoid nodes not behaving according to how the
protocols were originally set out. The absence of a \emph{deterministic}
policy for routing lookup requests and content-data avoids many outsiders exploring vulnerabilities
of deterministic predefined-defined policies;
\item \textbf{search/load balance:} in the absence of global knowledge, random search allows environment exploration
targeting opportunistic discovering of new resources. For problems involving choice between a number of known resources, 
such as communication links and source of contents, randomization can be used to spread the load among the resources. 
On the fly decisions allows load balance strategies to be applied, so to provide environment adaptability.
\end{enumerate}
These principles will be further discussed in the next chapter, where we introduce random walks. 







==> proposal.tex <==
\chapter{A Novel ICN Design}

\label{chapt:proposal}

Recall that in chapter 2, we have gone through a set of related works for Information
Centric Networks (ICN). We presented DONA solution and classified the others solutions
 in two main categories: $(i)$  DHT (distributed hash tables) and $(ii)$ BC (bread crumbs).
In this chapter, we introduce our novel design for an ICN architecture, focusing on content routing, 
searching and caching issues. We favor BC class of ICN solutions. 
   


\section{Routing/Caching}

Our design considers hierarchical \emph{tiers} composed of \emph{cache-routers}, $i.e.$, routers that can 
store content replicas. We define $k$ hierarchical levels.  Tier 1 is the top tier, and  tier $k$ is the bottom tier.  
Cache-routers in tier $k$ are connected to users. Published content, $i.e.$, contained maintained directly by the publishers, is stored in areas connected 
to cache-routers in tier $1$, 
through a TCP/IP network. 


We use flat names, with each content being hashed according to a hash-key. Storage areas are identified by hash-prefixes,
and are tuned for published content. For instance, if the hash prefix is 3 bit long, an storage area identified by the hash-prefix 
000 will only store hash-keys beginning with 000. More than one storage area can be assigned to the same hash prefix.
A random policy is applied in cache routers at tier $1$ to select, among the candidate storage areas, 
which one will serve a given lookup request.



Figure~\ref{tier11} shows the network organized in tiers. Two tiers $k$ are connected to the same tier $k-1$ in the
figure. Several tiers $k-1$ can be connected to the same tier $k-2$ and so on, up to tier $1$. A tier $1$ is connected to 
the storage areas through IP routers. Lookup requests that do not find content-data in cache-routers, while being routed 
towards a Tier $1$, are sent to the storage areas. Each tier, except tier $1$, has default cache-routers that connect to 
them at the next top level at the hierarchy, as shown in the figure.     




\begin{figure}
\center
\includegraphics[scale=0.4]{fig4_1}
\caption{Tiers and Storage Areas}
\label{system}
\label{tier11}
\end{figure}


In our design, the storage areas are not connected according to a pre-defined structure (topology). 
We do so in order to cope with the scalability and reliability issues discussed in chapter~\ref{chapt:icn}, 
related to (i) high maintenance overhead, (ii) topology disrupting for malicious attacks altering nodes operating according to 
predefined policies and (iii) concerns for published information being able to be managed on systems under the control of publisher 
trusted authorities. This implies that the search for a content in a storage area is done through a random
walk. Dominating sets, described in \textsection\ref{sec:global}, guide the walkers inside  the storage areas so as to 
assure that, in a finite number of steps,
a given content-data being searched among the nodes within a storage area will be found. Note also that  a published
content might be replicated more than once in a storage area.  The number of published copies, and their positions, are 
determined by a randomized algorithm, preventing external attacks that could 
hamper the reliability of storage areas, as discussed in \textsection\ref{sec:summaryopendesign}.


Lookup requests are sent from users towards storage areas, with each lookup request carrying a hash key 
for the corresponding content-data being searched. A copy of a lookup request is stored at
all the cache routers it traverses, being identified by the corresponding hash key and henceforth named bread crumb. 
This storage process sets a trail of bread crumbs towards storage areas. Reinforced counters (RCs) are assigned to bread crumbs when
initially stored. Each bread crumb is kept stored in a cache-router until its RC reaches zero. When a given lookup request traverses a 
given cache router, if there is already a bread crumb with the same hash-key stored in that cache router, the RC of the stored bread crumb is increased. 
After a pre-determined time since the last RC update of a bread crumb, the RC is decreased. When the RC of a bread crumb reaches 
zero value, it becomes invalid and is erased.



Figure~\ref{trailofbreadcrumbs} shows the setting of a trail of a bread crumb up to the storage areas. 
The violet arrows shows the flow of a lookup-request
from a user to the storage area. As a request traverse the cache-routers, a trail of bread crumbs is set, so content-data can be sent
to the user in the reverse path of the trail of bread crumbs. When the request reaches cache-routers in tier $1$, it is 
sent to the storage area through a retrieve primitive. Content-data inside the storage areas is encapsulated within the storage
area. The user never knows which node in a storage area will serve his request.



\begin{figure}
\center
\includegraphics[scale=0.4]{fig4_2}
\caption{Trail of bread crumbs}
\label{trailofbreadcrumbs}
\end{figure}



\marginpar{replication} When sent to users, content-data traverses a trail of bread crumbs in the reverse path, from the storage areas to users. 
The reinforce counter (RC) of all the corresponding content-data bread crumbs in the trail are checked out.  
If the RC of a stored bread crumb is above a certain $L$ threshold-level within a cache router, content-data is transferred from a
storage area to that cache router. Thus, whenever the popularity of a content is high, which means higher RCs for bread crumbs 
stored in cache routers, replica copies closer to the users should be provided. 




Figure~\ref{datastoragerouters} shows the transfer of a content-data from a storage area to a cache-router.  
The RC values of the bread crumbs at R1 and R2 are assumed to be greater than the threshold-level $L$.   The other RC values are assumed to be smaller than $L$. 
Therefore, \eat{after being requested by user 1. A} a replica of the content-data will be stored
in these cache-routers. \eat{ whose corresponding bread crumbs overpasses the $L$ threshold. Thus, i} In the other cache-routers 
\eat{ in the figure
that pertains to the same bread crumb trail,} no replica is stored. This avoids caching all requested contents close to users, in contrast to
 the caching policies deployed in BC ~\cite{elisha2}, BC+ ~\cite{bc+} and MCACHE ~\cite{multicache}, as described
in chapter 2. \emph{In our proposal, replica copies are transferred to cache-routers guided by the RC level, accounting for the popularity 
of the content-data being requested.}


\begin{figure}
\center
\includegraphics[scale=0.4]{fig4_3}
\caption{Data storage at cache routers}
\label{datastoragerouters}
\end{figure}



\marginpar{exploitation} Whenever a lookup-request is sent to the storage areas, the neighborhood of a cache-router in a tier is explored,
through \emph{biased random walks}, with $k$ explores, for a fixed amount of time. As the most popular contents are transferred from the storage areas
to the cache routers, the discovery of popular content-data is favored to take place at a cache-routers, instead of at storage areas.
As far as the discovery takes places in the neighborhood of a cache router, its forwarding tables can point to replicas in its neighborhood. 
\emph{Future requests for content data stored in cache-router tables can be sent directly to its neighborhood, 
according to a random load balance decision.  }



\section{Dominating Sets and Similarity Preferences}

\marginpar{random walks} When a lookup request arrives at a storage area, it does not have information about  which servers in their storage area 
have the content-data that is being looked for.  As there are no routing tables in storage areas,
content-data can be at any server. A random walk, involving multiples walkers, is performed to find the content-data. 
We assume that each storage area has up to $N$ servers. \eat{,  connected through a given topology. }
$N$ is upper bounded for the cover time of multiple random walks to be reasonable.

\marginpar{bias in storage areas} We intend to bias the walk inside an storage area marking
already visited nodes and its neighbors. We propose an algorithm, guided by dominant sets. 
Recall that a dominant set of a graph is a set of nodes such that each edge of the graph is 
incident to at least one node of the set (see \textsection\ref{sec:global}). 
The steps of the search algorithm inside each storage area are the following,
\begin{itemize}
\item \textbf{bootstrap:} We establish a vertex cover of the storage areas, through
bootstrapping;
\item \textbf{selection:} The walker selects a vertex not visited yet from the vertex
cover set, according to a uniform distribution;
\item \textbf{search:} The walker search for a content-data in the vertex selected
and its connected neighbors. If the content-data is not found, it marks
the selected vertex as visited and proceeds a new selection. If content-data is
found, the walker stops.
\end{itemize}


\marginpar{bias in cache-routers} We intend also to group replicas in cache routers according to similarities preferences. 
When a replica  is stored at a cache router, the hash-prefix of the content-data is announced throughout 
the cache-routers in a tier. This enables replicas in cache-routers to be clustered in tiers, according to hash-prefixes. 
Hash-prefixes are the features used to cluster content-data across cache-routers inside a tier (the approach could also be used across tiers).
When
an explorer intends to perform a random search for a content-data in a tier, it is guided by similarities within that tier.
In the same way that dominating sets operate as signal controls guiding random walks in storage areas, similarity preferences operate
as signal controls guiding random walks along cache-routers in a given tier. 

\begin{comment}

POR FAVOR, RELER E ESCREVER!!!


The above described replication policies decrease the load on the publishers and the amount of traffic sent to storage 
areas.   The topology connecting cache-routers within a tier has cache-routers at the edge 
with fewer degrees than 
the ones located at the center. This neighborhood exploitation is possible due to the announcement of a replica copy in a 
cache-router being sent to cache-routers in the same Tier, composing Similarity Preferences trails for guiding walks
within the network, as better described in the next section. None of the proposals reviewed in chapter 2 adopts this strategy,
that enhances the chance of finding a replica copy not pointed by a NRS, through randomness.


\end{comment}


\section{Challenges}


\subsection{Publish/subscribe Challenges} 

The policies for deciding in which storage area a given content-data will be stored and served must be defined. In particular, one needs to determine
\begin{itemize}
\item the number of nodes within a storage area;
\item the number of storage areas for each hash prefix and 
\item the topology that interconnects storage areas composing a cluster identified by the same hash prefix
\end{itemize} 


The adequate number of walkers and the number of dominating sets within a storage area, as well as the topology to interconnect 
the server nodes within a storage area,  pose additional challenges to be addressed in this thesis. It is our intention to explore 
topologies that allows a content-data with a given hash prefix associated not being stored at all storage areas handling that prefix.

It is our intention to explore topologies that cluster content-data 
in cache routers according to similarity preferences. For now, we consider similarity based on hash-prefixes. 
The granularity of hash-prefixes being announced at tiers is subject for research. Also, it is our desire to evaluate the effect 
of spreading storage areas along the tiers, so as to coordinate with the storage areas connected to tiers 1. 
The published information could be stored close to the users, as the replica copies.  


\subsection{Contet Distribution Challenges} 
How to set initial reinforced counters (RC) values for bread crumbs and how to update the RCs of stored
bread crumbs are also important open questions. The number of tiers, and the number of
cache-routers in each tier are also subject for investigation. 
The rules for load balancing to be used along cache-routers must also be defined. 
We intend to start with policies based on Ant Colony Optimization (ACO), and consider also other techniques. 



